Stochastic MPC with Multi-modal Predictions for Traffic Intersections

We propose a Stochastic MPC (SMPC) formulation for autonomous driving at traffic intersections which incorporates multi-modal predictions of surrounding vehicles for collision avoidance constraints. The multi-modal predictions are obtained with Gaussian Mixture Models (GMM) and constraints are formulated as chance-constraints. Our main theoretical contribution is a SMPC formulation that optimizes over a novel feedback policy class designed to exploit additional structure in the GMM predictions, and that is amenable to convex programming. The use of feedback policies for prediction is motivated by the need for reduced conservatism in handling multi-modal predictions of the surrounding vehicles, especially prevalent in traffic intersection scenarios. We evaluate our algorithm along axes of mobility, comfort, conservatism and computational efficiency at a simulated intersection in CARLA. Our simulations use a kinematic bicycle model and multimodal predictions trained on a subset of the Lyft Level 5 prediction dataset. To demonstrate the impact of optimizing over feedback policies, we compare our algorithm with two SMPC baselines that handle multi-modal collision avoidance chance constraints by optimizing over open-loop sequences.

==> Sections/conclusion.tex <==
% \section{Conclusion}
% \label{sec:conclusion}
% We proposed a SMPC formulation for EV control at traffic intersections, which uses GMMs for predicting TV trajectories for collision avoidance chance-constraints. The SMPC optimizes over a novel class of policies parameterised as a SOC, given by the sum of affine disturbance feedback over the EV's states and linear state feedback over the TV's states. % (granted by the causal structure \eqref{eq:TV_dyn_atv}).
% By exploiting additional structure in the GMM predictions, the proposed policy class is TV mode-agnostic for the first $\bar k-1$ time steps in the SMPC prediction horizon, and has separate mode-dependent policies for the remainder. The resulting SMPC optimization problem was shown to be a SOCP, which can be solved reliably and at approximately 20 Hz. Evaluating our algorithm against open-loop baselines along axes of mobility, comfort, conservatism and computational efficiency, we observed gains in mobility, comfort and efficiency while remaining significantly less conservative. 

==> Sections/proof.tex <==
\section{Proof of our ADF Policy Class being equivalent to state feedback} 
\subsection*{Setup: Models}
Let the LTV ego vehicle dynamics be given by 
\begin{align}\label{EV_dyn}
    \Delta x_{t+1}=A_t\Delta x_t+B_t\Delta u_t+w_t ~\forall t=0,\dots,N-1
\end{align}
where $w_t\sim\mathcal{N}(0,\Sigma_w)$.  The target vehicle dynamics be given by the switched ATV model
\begin{align}\label{TV_dyn}
    o_{t+1}=T_{t,\sigma_t}o_t+c_{t,\sigma_t}+n_{t}~\forall t=0,\dots, N-1
\end{align}
where $n_{t}\sim\mathcal{N}(0,\Sigma_n)$ and $\sigma_t\in\{1,\dots,J\}$ is the mode at time $t$.
Define the matrices $$\tilde{A}_{t,\sigma_t}=\begin{bmatrix}A_t&O\\O&T_{t,\sigma_t}\end{bmatrix}, \tilde{B}_{t}=\begin{bmatrix}B_t\\O\end{bmatrix}, \tilde{C}_{t,\sigma_t}=\begin{bmatrix}O\\c_{t,\sigma_t}\end{bmatrix}$$and stack the states and disturbances of \eqref{EV_dyn}, \eqref{TV_dyn} as $$\tilde{x}_t=\begin{bmatrix}\Delta x_t\\o_t\end{bmatrix},\ \tilde{w}_{t}=\begin{bmatrix}w_t\\n_{t}\end{bmatrix}.$$

The mode $\sigma_t$ is assumed unknown until some time $\bar t> 0$ in the future.

\begin{assumption}\label{assmp:tbar}
At time $\bar t> 0$, we can determine the mode $\sigma_{\bar t}$ from $o_{\bar t}$ and this mode is fixed for the remaining time steps, i.e., $\sigma_t=\sigma_{\bar t}~\forall t=\bar t, \dots, N-1$.
\end{assumption} 


Denote the mode sequence $\{\sigma_i\}_{i=0}^t$ by $\sigma_0^t$.
Given $\bar t$, define the set of admissible switching sequences as 
\begin{align}
    \mathcal{S}_{\bar t}=\{\hat\sigma_0^{N-1}\in\{1,\dots,J\}^N : \hat\sigma_t=\hat\sigma_{\bar t} ~\forall t\geq \bar t \}.
\end{align}
By assumption \ref{assmp:tbar}, the actual mode sequence $\sigma_0^{N-1}$ lies in this set, i.e., $\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$.


For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, let $\mathbf{x}^{\hat\sigma_0^{N-1}}=[\tilde{x}_0^\top\dots,\tilde{x}_N^\top]^\top$ be the states obtained by applying $\mathbf{u}=[\Delta u_0^\top\dots,\Delta u_{N-1}^\top]^\top$, as given by
\small
\begin{align}\label{eq:states_stacked}
\mathbf{x}^{\hat\sigma_0^{N-1}}=\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}_0+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{u}+\mathbf{C}^{\hat\sigma_0^{N-1}}+\mathbf{E}^{\hat\sigma_0^{N-1}}\mathbf{w}
\end{align}
\normalsize
where $\mathbf{w}=[\tilde{w}_0^\top\dots\tilde{w}_{N-1}^\top]^\top$, 

\scriptsize
\begin{align*}
    &\mathbf{A}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}I\\\tilde{A}_{0,\hat\sigma_0}\\\tilde{A}_{1,\hat\sigma_1}\tilde{A}_{0,\hat\sigma_0}\\\vdots\\\tilde{A}_{N-1,\hat\sigma_{N-1}}\hdots\tilde{A}_{0,\hat\sigma_0}\end{bmatrix},\\
    &\mathbf{C}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}O\\\tilde{C}_{0,\hat\sigma_0}\\\tilde{C}_{1,\hat\sigma_1}+\tilde{A}_{1,\hat\sigma_1}\tilde{C}_{0,\hat\sigma_0}\\\vdots\\\tilde{C}_{N-1,\hat\sigma_{N-1}}+\sum_{k=0}^{N-2}\tilde{A}_{N-1,\hat\sigma_{N-1}}\dots \tilde{A}_{k+1,\hat\sigma_{k+1}}\tilde{C}_{k,\hat\sigma_k}\end{bmatrix},\\
    &\mathbf{B}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}O&\hdots&\hdots& O\\\tilde{B}_{0}&O&\hdots&O\\\tilde{A}_{1,\hat\sigma_1}\tilde{B}_{0}&\tilde{B}_{1}&\hdots&O\\\vdots\\\tilde{A}_{N-1,\hat\sigma_{N-1}}\hdots\tilde{A}_{1,\hat\sigma_1}\tilde{B}_{0}&\hdots&\tilde{A}_{N-1,\hat\sigma_{N-1}}\tilde{B}_{N-2}&\tilde{B}_{N-1}\end{bmatrix},\\
    &\mathbf{E}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}O&\hdots&\hdots& O\\I&O&\hdots&O\\\tilde{A}_{1,\hat\sigma_1}&I&\hdots&O\\\vdots\\\tilde{A}_{N-1,\hat\sigma_{N-1}}\hdots\tilde{A}_{1,\hat\sigma_1}&\hdots&\tilde{A}_{N-1,\hat\sigma_{N-1}}&I\end{bmatrix}.
\end{align*}
\normalsize
\subsection*{Setup: Control Problem}
Given initial condition $\tilde{x}_0=\tilde{x}$, we seek feedback policies $\Delta u_t=\pi_t(\tilde{x}_t)~\forall t=0,\dots,N-1$ such that the following 
 obstacle avoidance constraints and input constraints are  satisfied by \eqref{EV_dyn}, \eqref{TV_dyn}: 
\begin{align}
    &\mathbb{P}(\mathbf{H}\mathbf{x}^{\sigma_0^{N-1}}\leq \mathbf{h}\ |\tilde{x}_0=\tilde{x} )\geq p,\\
    &\mathbb{P}(\mathbf{G}\mathbf{u}^{\sigma_0^{N-1}}\leq \mathbf{g}\ |\tilde{x}_0=\tilde{x})\geq p
\end{align}
where $\mathbf{u}^{\sigma_0^{N-1}}=[\pi_0(\tilde{x}_0)^\top\dots\pi_{N-1}(\tilde{x}_{N-1})^\top]^\top$ and $\mathbf{H}, \mathbf{G}$ have $n_H$ and $n_G$ rows respectively. 
Note that $\sigma_0^{N-1}$ is not known at $t=0$, and thus we look for policies $\pi_t(\cdot)$ such that
\begin{align}\label{control_problem}
    &\mathbb{P}(\mathbf{H}\mathbf{x}^{\hat\sigma_0^{N-1}}\leq \mathbf{h}\ |\tilde{x}_0=\tilde{x} )\geq p,\nonumber\\
    &\mathbb{P}(\mathbf{G}\mathbf{u}^{\hat\sigma_0^{N-1}}\leq \mathbf{g}\ |\tilde{x}_0=\tilde{x})\geq p~~ \forall\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}.
\end{align}
\subsection*{Policy Candidates}
\subsubsection{Affine state feedback policy class}

Consider the following control policy
\small
\begin{align}\label{eq:ASF}
    \pi^{ASF}_{t}(\tilde{x}_t)=\begin{cases}
    \sum_{k=0}^tK_{k,t}\tilde{x}_k+v_t, &\text{for } t<\bar t\\
    \sum_{k=0}^tK^{1}_{k,t}\tilde{x}_k+v^{1}_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=1\\
    \vdots & \vdots\\
    \sum_{k=0}^tK^{J}_{k,t}\tilde{x}_k+v^{J}_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=J
    \end{cases}
\end{align}
\normalsize
In view of assumption \ref{assmp:tbar}, this policy is mode-agnostic for $t<\bar t$ and mode-dependent for $t\geq \bar t$.
For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, define 
\scriptsize
$$\mathbf{v}^{\hat\sigma_{\bar t}}=[v_0^\top\dots v_{\bar t-1}^\top\  v^{\hat\sigma_{\bar t}\top}_{\bar t}\dots v^{\hat\sigma_{\bar t}\top}_{N-1}]^\top, $$
\begin{align*}
    \mathbf{K}^{\hat\sigma_{\bar t}}=\begin{bmatrix}K_{0,0}&O&\hdots&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K_{0,\bar t-1}&\hdots K_{\bar t-1,\bar t-1}&O&\hdots& O\\
    K^{\hat\sigma_{\bar t}}_{0,\bar t}&\hdots &K^{\hat\sigma_{\bar t}}_{\bar t,\bar t}&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K^{\hat\sigma_{\bar t}}_{0,N-1}&\hdots &\hdots& K^{\hat\sigma_{\bar t}}_{N-1,N-1}&O
    \end{bmatrix}
\end{align*}
\normalsize
to get 
\begin{align}\label{eq:ASF_control_stacked}
\mathbf{u}_{ASF}^{\hat\sigma_0^{N-1}}=\mathbf{K}^{\hat\sigma_{\bar t}}\mathbf{x}_{ASF}^{\hat\sigma_0^{N-1}}+\mathbf{v}^{\hat\sigma_{\bar t}}.
\end{align}
where $\mathbf{x}_{ASF}^{\hat\sigma_0^{N-1}}$ is the closed-loop trajectory given by substituting \eqref{eq:ASF_control_stacked} in \eqref{eq:states_stacked}. The closed-loop trajectory can be given in closed-form as 
\small
\begin{align}\label{eq:ASF_stacked_states}
    \mathbf{x}^{\hat\sigma_0^{N-1}}_{ASF}=&(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}(\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}_0+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{v}^{\hat\sigma_{\bar t}}+\mathbf{C}^{\hat\sigma_0^{N-1}})\nonumber\\&+(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}\mathbf{E}^{\hat\sigma_0^{N-1}}\mathbf{w}
\end{align}
\normalsize
where the matrix $\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}}$ can be shown to be lower triangular with all diagonal entries being $1$, and thus, invertible. Note that due to the presence of the inverse $(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}$, the closed-loop states $\mathbf{x}^{\hat\sigma_0^{N-1}}_{ASF}$ are generally nonlinear functions of $\mathbf{K}^{\hat\sigma_{\bar t}},\ \mathbf{v}^{\hat\sigma_{\bar t}}$. 


For given $\hat\sigma_0^{N-1}$ and $ \mathbf{K}^{\hat\sigma_{\bar t}}, \mathbf{v}^{\hat\sigma_{\bar t}}$, the chance constraints \eqref{control_problem} can be tightened as follows. 
\footnotesize
\begin{align}\label{state_chance_constr_tightened}
    &\mathbb{P}(\mathbf{H}_i\mathbf{x}_{ASF}^{\hat\sigma_0^{N-1}}>\mathbf{h}_i |\tilde{x}_0=\tilde{x})\leq\frac{1-p}{n_H}~\forall i=1,\dots,n_H\nonumber\\
    \Leftrightarrow&\mathbf{H}_i(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}(\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{v}^{\hat\sigma_{\bar t}}+\mathbf{C}^{\hat\sigma_0^{N-1}})\nonumber\\
    &~~+\text{cdf}^{-1}\left(p_H\right)\Vert\mathbf{H}_i(\mathbf{I}-\mathbf{B}^\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}\mathbf{E}^{\hat\sigma_0^{N-1}}\Sigma_{\tilde{w}}^{\frac{1}{2}}\Vert\leq\mathbf{h}_i\nonumber\\
    &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\forall i=1,\dots,n_H
\end{align}
\begin{align}\label{input_chance_constr_tightened}
    &\mathbb{P}(\mathbf{G}_j\mathbf{u}_{ASF}^{\hat\sigma_0^{N-1}}>\mathbf{g}_j|\tilde{x}_0=\tilde{x})\leq\frac{1-p}{n_G}~\forall j=1,\dots,n_G\nonumber\\
    \Leftrightarrow&\mathbf{G}_j(\mathbf{K}^{\hat\sigma_{\bar t}}(\mathbf{I}-\mathbf{B}^\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}(\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{v}^{\hat\sigma_{\bar t}}+\mathbf{C}^{\hat\sigma_0^{N-1}})+\mathbf{v}^{\hat\sigma_{\bar t}})\nonumber\\&~~+\text{cdf}^{-1}\left(p_G\right)\Vert\mathbf{G}_j\mathbf{K}^{\hat\sigma_{\bar t}}(\mathbf{I}-\mathbf{B}^\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}\mathbf{E}^{\hat\sigma_0^{N-1}}\Sigma_{\tilde{w}}^{\frac{1}{2}}\Vert\leq\mathbf{g}_j\nonumber\\
    &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\forall j=1,\dots,n_G
\end{align}
\normalsize
where cdf$^{-1}(\cdot)$ is the inverse of the cumulative distribution function of $\mathcal{N}(0,1)$, $p_H=1-\frac{1-p}{n_H}$, $p_G=1-\frac{1-p}{n_G}$ and $\Sigma_{\tilde{w}}=\begin{bmatrix}\Sigma_w&O\\O&\Sigma_n\end{bmatrix}$.


For a given initial condition $\tilde{x}_0=\tilde{x}$, an inner approximation of the class of affine state feedback policies of the form \eqref{eq:ASF} that satisfies \eqref{control_problem} is given by the set
\begin{align}
    \Pi_{ASF}(\tilde{x})=\{\{\mathbf{K}^j,\mathbf{v}^j\}_{\forall j\in\{1,\dots,J\}}:\eqref{state_chance_constr_tightened},\eqref{input_chance_constr_tightened}~ \forall \hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}\ \}
\end{align}
\subsubsection{Affine switched disturbance feedback policy class:}
For any $\hat\sigma_{0}^{N-1}\in\mathcal{S}_{\bar t}$ and any $t\geq 1$, we can use measurements $\tilde{x}_t, \tilde{x}_{t-1}$ and $\Delta u_{t-1}$ to define $$\tilde{w}_{t-1,\hat\sigma_{t-1}}=\tilde{x}_{t}-\tilde{A}_{t-1,\hat\sigma_{t-1}}\tilde{x}_{t-1}-\tilde{B}_{t-1}\Delta u_{t-1}-\tilde{C}_{t-1,\hat\sigma_{t-1}}.$$ 
 For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, let
\small
\begin{align}\label{eq:ADF_sigma}
    &u^{\hat\sigma_0^{N-1}}_{t}=\begin{cases}
    \sum_{k=0}^{t-1}M_{k,t}\begin{bmatrix}w_{k}\\n_{k,\hat\sigma_k}\end{bmatrix}+h_t, &\text{for } t<\bar t\\
    M^1_{k,t}\begin{bmatrix}w_{k}\\n_{k,\hat\sigma_k}\end{bmatrix}+h^1_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=1\\
    \vdots & \vdots\\
    M^J_{k,t}\begin{bmatrix}w_{k}\\n_{k,\hat\sigma_k}\end{bmatrix}+h^J_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=J
    \end{cases}
\end{align}
\normalsize
and define the feedback control policy as
\begin{align}\label{eq:ADF}
    \pi^{ASDF}(\tilde{x}_t)\in\{u^{\hat\sigma_0^{N-1}}_{t}\}_{\forall\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}}
\end{align}
Like \eqref{eq:ASF}, this policy is mode agnostic for $t<\bar t$ and mode-dependent for $t\geq \bar t$. However, this policy is non-deterministic except at $t=0$ when $\pi^{ASDF}_0(\tilde{x}_0)=h_0$.

For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, define 
\scriptsize
$$\mathbf{h}^{\hat\sigma_{\bar t}}=[h_0^\top\dots h_{\bar t-1}^\top\  h^{\hat\sigma_{\bar t}\top}_{\bar t}\dots h^{\hat\sigma_{\bar t}\top}_{N-1}]^\top, $$
\begin{align*}
    \mathbf{M}^{\hat\sigma_{\bar t}}=\begin{bmatrix}
    O&\hdots&\hdots&\hdots& O\\M_{0,1}&O&\hdots&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K_{0,\bar t-1}&\hdots K_{\bar t-1,\bar t-1}&O&\hdots& O\\
    K^{\hat\sigma_{\bar t}}_{0,\bar t}&\hdots &K^{\hat\sigma_{\bar t}}_{\bar t,\bar t}&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K^{\hat\sigma_{\bar t}}_{0,N-1}&\hdots &\hdots& K^{\hat\sigma_{\bar t}}_{N-1,N-1}&O
    \end{bmatrix}
\end{align*}
\normalsize

